How Effectively Do Security Skills Guide Coding Agents in Vulnerability Detection in Linux Kernel?

Large language model (LLM) coding agents, such as Claude Code, are increasingly used for security auditing, with task-specific skills providing reusable vulnerability-analysis procedures. However, their effectiveness in detecting real vulnerabilities and the reasons for their failures remain unclear. We conduct the first large-scale empirical study of 37 security skills using Claude Code with four underlying LLMs on 100 real Linux kernel vulnerabilities across ten classes, totaling 14800 runs. We evaluate vulnerability detection at the function, statement, and vulnerability-class levels. Results show that 24.4 percent of runs locate the correct function, 18.3 percent identify both the function and responsible statement, and 15.7 percent correctly classify the vulnerability. Our failure analysis reveals limitations in evidence acquisition, state-relation reasoning, code interpretation, candidate verification, investigation coverage, and reporting. Based on these findings, we propose SKILL-SIF, a self-improving framework that iteratively evolves security skills by learning from missed vulnerabilities and failure patterns. We evolve five top-performing skills using the original benchmark and evaluate them on 100 previously unseen vulnerabilities. SKILL-SIF improves fully correct vulnerability detection by up to eight times (from 2 percent to 16 percent) on unseen vulnerabilities, while aggregate accuracy across four LLMs increases by 1.85 times (from 6.05 percent to 11.20 percent). These findings highlight the limitations of existing security skills and demonstrate the potential of failure-driven skill evolution to improve vulnerability detection in coding agents.

==> figure/cwe_detection_comparion.tex <==
\begin{figure*}[t]
  \centering  
  \includegraphics[
  width=0.98\textwidth,
  height=0.3\textheight
]{figure/cwe_detection_comparison.png}
 
  \caption{Localization and vulnerability detection performance across CWE classes. Markers show the percentages of runs identifying the responsible function, both the function and statement, and all three required elements: vulnerability class, function, and statement. Percentages use 1,480 runs per CWE. Lines connect the three criteria, and classes are ordered by the fully correct rate.\song{resolution is low}}
  \label{fig:cwe-detetcion-com}
\end{figure*}



==> figure/m2_example.tex <==
\begin{figure*}[t!]
  \centering  \includegraphics[width=\textwidth,
  height=6cm,
    keepaspectratio]
    {figure/Code Timeout Path and DMA Buffer Analysis (1).png}
   % \vspace{-0.8cm}
  \caption{Example of M2 - the agent identifies the timeout path and the buffer free, but does not connect them through the hardware ownership relation, and therefore misses the user-after-free vulnerability. } 
\label{fig:m2_example}
% \vspace{-0.7cm}

\end{figure*}

==> figure/m3_example.tex <==
\begin{figure*}[t!]
  \centering  \includegraphics[width=\textwidth,
  height=6cm,
    keepaspectratio]
    {figure/IRQ Domain Cleanup Analysis Diagram.png}
   % \vspace{-0.8cm}
  \caption{Example of M3 - the agent does inspect the relevant cleanup path, but then makes the specific incorrect assumption that removing the IRQ domain also releases the generic IRQ-chip resources. } 
\label{fig:m3_example}
% \vspace{-0.7cm}

\end{figure*}

==> figure/refine_example.tex <==
\begin{figure*}[t!]
  \centering  \includegraphics[width=\textwidth,
  height=6cm,
    keepaspectratio]
    {figure/Skill-Guided Code Analysis Comparison.png}
   % \vspace{-0.8cm}
  \caption{Example of skill-level limitation removed through skill refinement. The original skill misses the target failure path, causing investigation and coverage gap limitation, while the refined skill explicitly guides the agent to inspect it and localize the defect. } 
\label{fig:s4_example}
\vspace{-0.3cm}

\end{figure*}

==> figure/s4_example.tex <==
\begin{figure*}[t!]
  \centering  \includegraphics[width=\textwidth,
  height=6cm,
    keepaspectratio]
    {figure/Checklist Gap Behind Missed Concurrency Bug.png}
   % \vspace{-0.8cm}
  \caption{Example of S4 - The run replaces the intended checklist procedure with a generic review, and the target timer/refcount ordering analysis is never performed. } 
\label{fig:s4_example}
\vspace{-0.5cm}

\end{figure*}

==> sec/background.tex <==
\section{Background and Related Work}
\label{sec:background}



==> sec/lessons.tex <==
\section{Lessons Learned}
\label{sec:lessons}




==> tabs/MethodTechiniqueCategory.tex <==
\begingroup
\footnotesize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.7}

\begin{longtable}{
    >{\raggedright\arraybackslash}p{1.05cm}
    >{\raggedright\arraybackslash}p{3.8cm}
    >{\raggedright\arraybackslash}p{8.0cm}
    >{\raggedleft\arraybackslash}p{0.9cm}
}
\caption{Methods and Techniques Categories of Security Skills}
\label{tab:methods-techniques-categories} \\

\toprule
\textbf{ID} &
\textbf{Methods/Techniques Category} &
\textbf{Marker/Evidence Used for Assignment} &
\textbf{Count} \\
\midrule
\endfirsthead

\multicolumn{4}{c}%
{{\tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{ID} &
\textbf{Methods/Techniques Category} &
\textbf{Marker/Evidence Used for Assignment} &
\textbf{Count} \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot

MTC-01 &
LLM-Native Static Reasoning &
Instructs the model to inspect code and reason with built-in security patterns or rubrics, without running external tools. &
1,477 \\

MTC-02 &
External Security-Tool Orchestration &
Runs named security tools such as Semgrep, CodeQL, Bandit, Trivy, Checkov, Slither, Nuclei, SQLMap, or Nmap and interprets their results. &
1,401 \\

MTC-03 &
Pattern / Regex / AST Grep Scanning &
Scans code using grep, ripgrep, ast-grep, or custom regex/pattern rules as the primary mechanism. &
435 \\

MTC-04 &
Manifest \& Advisory-Database Lookup &
Reads manifests or lockfiles and checks dependencies against advisory sources such as NVD, GHSA, OSV, npm audit, or pip-audit. &
295 \\

MTC-05 &
Dynamic Probing \& Active Exploitation &
Interacts with a live target using requests, payloads, exploits, browsers, or proxies to trigger and observe security-relevant behavior. &
1,510 \\

MTC-06 &
Fuzzing \& Property-Based Testing &
Generates mutated or randomized inputs to trigger faults using fuzzers or property/invariant testing. &
88 \\

MTC-07 &
Binary Instrumentation \& Reverse Engineering &
Uses disassemblers, debuggers, instrumentation, or sanitizers, such as Ghidra, radare2, GDB, or Frida, for analysis. &
232 \\

MTC-08 &
Configuration \& Policy Compliance Evaluation &
Parses configuration, IaC, or cloud-state artifacts and checks them against security rules, policies, or benchmarks. &
181 \\

MTC-09 &
Checklist / Framework-Driven Review &
Reviews a target systematically using a structured standard, framework, or control checklist such as OWASP ASVS, CIS, NIST, or SOC 2. &
397 \\

MTC-10 &
Threat Modelling \& Architectural Analysis &
Analyzes data flows, trust boundaries, and attack paths to derive threats from system architecture rather than artifact scanning. &
126 \\

MTC-11 &
Multi-Agent / Pipeline Orchestration &
Uses multiple sub-agents or specialized analysis phases as the defining workflow. &
228 \\

MTC-12 &
Bundled Custom Analyzer Scripts &
Ships and runs its own analyzer scripts, such as Python or shell scripts, that perform the core analysis. &
491 \\

MTC-13 &
Log, Telemetry \& Detection-Rule Analysis &
Analyzes logs, events, or telemetry, or creates detection content such as YARA, Sigma, or SIEM rules. &
290 \\

MTC-14 &
Reference / Advisory Knowledge Delivery &
Provides curated security knowledge, patterns, or remediation guidance without performing target-specific analysis. &
104 \\

MTC-15 &
API / Platform Data Integration &
Uses vendor or platform APIs, such as Snyk, GitHub Security, Dependabot, or cloud-security services, as the primary analysis mechanism. &
212 \\

\end{longtable}

\endgroup

==> tabs/PrimaryfunctionalCategory.tex <==
\begingroup
\footnotesize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.7}

\begin{longtable}{
    >{\raggedright\arraybackslash}p{1.05cm}
    >{\raggedright\arraybackslash}p{3.6cm}
    >{\raggedright\arraybackslash}p{8.2cm}
    >{\raggedleft\arraybackslash}p{0.9cm}
}
\caption{Primary Functional Categories of Security Skills}
\label{tab:primary-functional-categories} \\

\toprule
\textbf{ID} &
\textbf{Primary Functional Category} &
\textbf{What It Covers} &
\textbf{Count} \\
\midrule
\endfirsthead

\multicolumn{4}{c}%
{{\tablename\ \thetable{} -- continued from previous page}} \\
\toprule
\textbf{ID} &
\textbf{Primary Functional Category} &
\textbf{What It Covers} &
\textbf{Count} \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot

PFC-01 &
Source Code Vulnerability Detection &
Reviews first-party source code for injection, authentication, cryptographic, memory, and logic flaws using OWASP/CWE-style audits or scanners; excludes dependency and infrastructure checks. &
1,675 \\

PFC-02 &
Dependency \& Supply-Chain Security &
Examines third-party dependencies for known CVEs, malicious or typosquatted packages, SBOM/provenance risks, license issues, and lockfile integrity. &
506 \\

PFC-03 &
Secrets \& Credential Exposure Detection &
Detects hardcoded or leaked keys, tokens, and passwords in source code or Git history, with supporting triage and rotation workflows. &
163 \\

PFC-04 &
Infrastructure, Cloud \& Container Security Posture &
Checks IaC, containers, cloud environments, CI/CD pipelines, and repository settings for security misconfigurations and hardening issues. &
492 \\

PFC-05 &
Web \& API Application Security Testing &
Actively tests running web applications and APIs through DAST, endpoint fuzzing, IDOR/SSRF/XSS probing, and authentication-flow attacks. &
1,181 \\

PFC-06 &
Offensive Security \& Exploitation &
Covers penetration testing, reconnaissance, privilege escalation, exploitation, post-exploitation, exploit development, CTFs, and bug-bounty workflows. &
823 \\

PFC-07 &
Smart Contract \& Blockchain Security &
Audits smart contracts and blockchain protocols for reentrancy, economic attacks, chain-specific vulnerabilities, and DeFi risks. &
179 \\

PFC-08 &
AI/LLM \& Agent Security &
Assesses prompt injection, jailbreaks, OWASP LLM risks, agent/tool permissions, MCP configurations, and model supply-chain security. &
396 \\

PFC-09 &
Threat Modeling \& Security Design Review &
Analyzes architectures and data flows using threat models, trust boundaries, and attack trees to derive threats, abuse cases, and security requirements. &
147 \\

PFC-10 &
Compliance, Governance \& Standards Auditing &
Assesses security-control gaps and evidence against standards and regulations such as SOC 2, PCI DSS, HIPAA, GDPR, NIST, CIS, and ISO 27001. &
157 \\

PFC-11 &
Vulnerability Management \& Triage &
Prioritizes existing findings using CVE/CVSS/EPSS data, monitoring, deduplication, false-positive triage, patch planning, and reporting; excludes initial discovery. &
432 \\

PFC-12 &
Malware, Threat Detection, IR \& Forensics &
Covers malware and backdoor analysis, YARA/IOC detection, digital forensics, incident response, threat hunting, and SOC workflows. &
776 \\

PFC-13 &
Secure Development Guidance \& Remediation &
Provides secure-coding, hardening, and remediation guidance for known vulnerability classes; focuses on prevention and fixing rather than discovery. &
36 \\

PFC-14 &
Binary, Reverse Engineering \& Memory Safety &
Uses reverse engineering, instrumentation, sanitizers, and fuzzing to analyze binaries, firmware, protocols, and memory-corruption vulnerabilities. &
210 \\

PFC-15 &
Mobile Application Security &
Assesses Android and iOS applications through MASVS review, pinning/root/jailbreak bypass, component and deep-link testing, and static/dynamic analysis. &
136 \\

PFC-16 &
Network \& Protocol Security Assessment &
Assesses services, TLS/certificates, wireless and network protocols, firewalls/WAFs, and DNS/email security posture. &
169 \\

\end{longtable}

\endgroup

==> tabs/co-occurrence.tex <==
\begin{table}[t]
\centering
\caption{Most common mismatch co-occurrence patterns. Sink and root-cause fields are proxy comparisons derived from changed statements.}
\label{tab:failure-cooccurrence}
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc}
\toprule
Mismatch pattern & Count \\
\midrule
CWE + function + line + statement + sink + root cause & 1451 \\
Function + line + statement + sink + root cause & 310 \\
CWE + line + statement + sink + root cause & 70 \\
CWE + function + line + statement + sink & 50 \\
CWE + sink only & 50 \\
Sink only & 47 \\
No mismatch on core/proxy fields & 45 \\
Line + statement + sink + root cause & 37 \\
CWE only & 27 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tabs/cwe_performance.tex <==
\begin{table}[t]
\centering
\caption{Vulnerability detection and localization performance by CWE}
\label{tab:cwe_performance}
\begin{tabular}{lrrrr}
\toprule
\textbf{CWE} & \textbf{Function Localized} & \textbf{Function + Statement} & \textbf{Fully Correct} & \textbf{Correct (\%)} \\
\midrule
CWE-416                 & 289 & 201 & 172 & 11.62 \\
CWE-476          & 350 & 284 & 215 & 14.53 \\
CWE-401          & 231 & 168 & 56  & 3.78  \\
CWE-125                 & 667 & 550 & 432 & 29.19 \\
CWE-787               & 981 & 921 & 585 & 39.53 \\
CWE-667                  & 129 & 26  & 6   & 0.41  \\
CWE-908       & 237 & 140 & 29  & 1.96  \\
CWE-825       & 254 & 138 & 60  & 4.05  \\
CWE-362           & 196 & 123 & 51  & 3.45  \\
CWE-617               & 276 & 150 & 32  & 2.16  \\
\bottomrule
\end{tabular}
\end{table}

==> tabs/dominant_confusion.tex <==
\begin{table}[t]
  \centering
  \caption{Dominant wrong-CWE transitions across all skills.}
  \label{tab:dominant-confusions}
  % \scriptsize
  \begin{tabular}{lc}
  \toprule
  Ground truth $\rightarrow$ reported CWE & Count \\
  \midrule
  CWE-416 $\rightarrow$ CWE-476 & 172 \\
  CWE-476 $\rightarrow$ CWE-125 & 97 \\
  CWE-476 $\rightarrow$ CWE-190 & 88 \\
  CWE-416 $\rightarrow$ CWE-125 & 67 \\
  CWE-476 $\rightarrow$ CWE-416 & 61 \\
  CWE-416 $\rightarrow$ CWE-190 & 61 \\
  CWE-476 $\rightarrow$ CWE-787 & 50 \\
  CWE-125 $\rightarrow$ CWE-190 & 47 \\
  CWE-125 $\rightarrow$ CWE-787 & 43 \\
  CWE-787 $\rightarrow$ CWE-476 & 41 \\
  \bottomrule
  \end{tabular}%
  \end{table}

==> tabs/failure_taxonomy_update.tex <==
\begin{landscape}
\begin{table*}[t]
\centering
\caption{Validated failure taxonomy with representative examples.
Each example briefly summarizes the failure cases and reasons.}
\label{tab:failure_taxonomy_examples}

\scriptsize
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{0.92}

\begin{tabularx}{\linewidth}{
>{\raggedright\arraybackslash}p{1.0cm}
>{\raggedright\arraybackslash}p{4.0cm}
>{\raggedright\arraybackslash}X
@{\hspace{7pt}}
>{\raggedright\arraybackslash}p{1.0cm}
>{\raggedright\arraybackslash}p{4.0cm}
>{\raggedright\arraybackslash}X
}
\toprule

\multicolumn{3}{c}{\textbf{Agent Execution Failures}} &
\multicolumn{3}{c}{\textbf{Skill-Level Limitations}} \\

\cmidrule(r){1-3}
\cmidrule(l){4-6}

\textbf{ID} &
\textbf{Description} &
\textbf{Representative Example} &
\textbf{ID} &
\textbf{Description} &
\textbf{Representative Example} \\

\midrule

\textbf{M1} &
Relevant evidence is not meaningfully analyzed. &
\textbf{IRQ-chip cleanup, model: haiku-4.5.}
Driver removal must release generic IRQ-chip resources before removing
their IRQ domain. The run instead focuses on unrelated interrupt logic and
\textbf{never analyzes the remove path or required cleanup}. &

\textbf{S1} &
The skill scope does not adequately adapt to the target task. &
\textbf{Kernel callback deadlock, skill: sc-race-condition.}
Teardown cancels a callback while holding a lock required by that callback.
The skill focuses on application-level races and provides
\textbf{no adaptation procedure for this kernel lock/callback relation}. \\

\addlinespace[1pt]

\textbf{M2} &
Relevant operations are found but the unsafe state relation is not constructed. &
\textbf{DMA lifetime, model: deepseek-v4-pro.}
A timeout may occur while hardware still owns the DMA buffer, which the
caller then frees. The run misses
\textbf{timeout $\rightarrow$ outstanding command $\rightarrow$ free
$\rightarrow$ later hardware access}. &

\textbf{S2} &
The skill lacks the kernel-specific state reasoning required by the target. &
\textbf{DMA lifetime, skill: abstract-state-analyzer.}
The skill models interval, null, sign, and type states but provides
\textbf{no procedure for tracking outstanding device ownership and safe release}. \\

\addlinespace[1pt]

\textbf{M3} &
An API, helper, state, lock, or execution contract is interpreted incorrectly. &
\textbf{IRQ-chip cleanup, model: deepseek-v4-pro.}
The run inspects the remove path but concludes that
irq\_domain\_remove() \textbf{``will also free the generic chips''}, which misinterprets the cleanup contract. &

\textbf{S3} &
The skill lacks sufficient investigation or coverage rules. &
\textbf{Stored \texttt{mm} lifetime, skill: memory-api-misuse.}
Safety requires following the separately stored \texttt{mm} object through
later use and destruction, but the skill explicitly performs
\textbf{local rather than whole-program lifetime analysis}. \\

\addlinespace[1pt]

\textbf{M4} &
A conclusion is unsupported, contradicted, or stronger than the evidence permits. &
\textbf{Packet-pointer lifetime, model: sonnet-5.}
The run proves sufficient packet bounds but uses that result to conclude
\textbf{pointer-lifetime safety}, without resolving whether later buffer
relocation invalidates the saved pointer. &

\textbf{S4} &
The skill depends on an unavailable resource without an effective alternative. &
\textbf{Timer/refcount ordering, skill: workerd-safety-review.}
The skill requires an external safety checklist, but the run reports
\textbf{``the checklist file doesn't exist''} and falls back to a generic review. \\

\addlinespace[1pt]

\textbf{M5} &
A relevant candidate is closed before the decisive question is resolved. &
\textbf{Stale IOMMU pointer, model: sonnet-5.}
The run identifies a stale \texttt{group->domain} pointer but records
\textbf{\texttt{verdict: dropped}} before determining whether it can later
be used after free. &

\textbf{S5} &
The skill lacks a sufficient evidence-verification or completion rule. &
\textbf{DMA lifetime, skill: abstract-state-analyzer.}
The workflow reaches reporting without explicitly requiring unresolved
timeout/free interactions to be challenged, allowing
\textbf{an unverified safety conclusion to survive}. \\

\addlinespace[1pt]

\textbf{M6} &
An available investigation step is carried out ineffectively. &
\textbf{Work-cancellation deadlock, model: deepseek-v3.2.}
After recognizing \textbf{``I'm missing the path parameter''}, the run
repeats unrelated searches rather than tracing
cancel\_work\_sync(), its callback, and the held mutex. &

\textbf{S6} &
The skill permits unresolved candidates to be discarded during triage. &
\textbf{Stale IOMMU pointer, skill: forge-bughunter.}
The skill applies a \textbf{``prove it or drop it''} rule, and the candidate
is discarded before its later-use condition is resolved. \\

\addlinespace[1pt]

\textbf{M7} &
A supported finding is altered or lost before final reporting. &
\textbf{Reachable kernel assertion, model: deepseek-v3.2.}
The intermediate analysis identifies the relevant
BUG\_ON, but \textbf{the finding disappears from the final artifact}. &

\textbf{S7} &
The skill handoff does not preserve all information required by the final task. &
\textbf{Reachable kernel assertion, skill: sast-flow-tracer.}
The skill outputs an intermediate flow artifact, and
\textbf{the relevant vulnerability flow is not preserved in the final handoff}. \\

\bottomrule
\end{tabularx}

\end{table*}
\end{landscape}

==> tabs/localization.tex <==
\begin{table}[t]
\centering
\caption{Localization and correctness performance by model.}
\label{tab:model_localization}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccc}
\toprule
\textbf{Model} &
\makecell{\textbf{Function}\\\textbf{Localized}} &
\makecell{\textbf{Function + Statement}\\\textbf{Localized}} &
\textbf{Correct} &
\makecell{\textbf{Function} $\rightarrow$\\\textbf{Statement}} &
\makecell{\textbf{Locations} $\rightarrow$\\\textbf{Correct}} \\
\midrule

Claude Haiku-4.5
& 767 (20.73\%)
& 545 (14.73\%)
& 205 (5.54\%)
& 71.06\%
& 37.61\% \\

Claude Sonnet-5
& 980 (26.49\%)
& 693 (18.73\%)
& 473 (12.78\%)
& 70.71\%
& 68.25\% \\

DeepSeek-V3.2
& 577 (15.59\%)
& 395 (10.68\%)
& 213 (5.76\%)
& 68.46\%
& 53.92\% \\

DeepSeek-V4-Pro
& 1,286 (34.76\%)
& 1,068 (28.86\%)
& 747 (20.19\%)
& 83.05\%
& 69.94\% \\

\midrule
\textbf{All models}
& \textbf{3,610 (24.39\%)}
& \textbf{2,701 (18.25\%)}
& \textbf{1,638 (11.07\%)}
& \textbf{74.82\%}
& \textbf{60.64\%} \\

\bottomrule
\end{tabular}
\end{table}

==> tabs/overall_model.tex <==
\begin{table}[t]
\centering
\caption{Model performance and vulnerability coverage.}
\label{tab:model_performance}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Model} & \textbf{Fully Correct} & \textbf{Partial} & \textbf{Incorrect} & \textbf{Correct (\%)} & \textbf{Vulnerabilities Covered} \\
\midrule
Claude Haiku-4.5 & 205 & 692 & 2,803 & 5.54 & 37/100 \\
Claude Sonnet-5 & 473 & 591 & 2,636 & 12.78 & 41/100 \\
DeepSeek-V3.2 & 213 & 582 & 2,905 & 5.76 & 32/100 \\
DeepSeek-V4-Pro & 747 & 757 & 2,196 & 20.19 & 59/100 \\
\midrule
\textbf{All models} & \textbf{1,638} & \textbf{2,622} & \textbf{10,540} & \textbf{11.07} & \textbf{64/100} \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[t] 
% \centering 
% \caption{Overall effectiveness of skills on the 266-case evaluation set.} \label{tab:overall-effectiveness} \scriptsize \setlength{\tabcolsep}{5pt} \renewcommand{\arraystretch}{0.9} \setlength{\aboverulesep}{0.25ex} \setlength{\belowrulesep}{0.25ex} \begin{tabular}{@{}lrrrrrrrr@{}} \toprule \textbf{Skill} & \textbf{TP} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} & \textbf{FPR} & \textbf{Func.} & \textbf{Line} & \textbf{Stmt.} \\ \midrule vulnHunter & 60 & 0.455 & 0.226 & 0.302 & 0.068 & 0.150 & 0.086 & 0.083 \\ Semgrep & 67 & 0.416 & 0.252 & 0.314 & 0.088 & 0.132 & 0.071 & 0.071 \\ code-quality & 61 & 0.415 & 0.229 & 0.295 & 0.081 & 0.143 & 0.086 & 0.086 \\ sast & 43 & 0.361 & 0.162 & 0.223 & 0.071 & 0.150 & 0.079 & 0.068 \\ sast-config. & 63 & 0.426 & 0.237 & 0.304 & 0.080 & 0.135 & 0.090 & 0.086 \\ security-reviewer & 60 & 0.423 & 0.226 & 0.294 & 0.077 & 0.128 & 0.090 & 0.083 \\ cybersecurity & 56 & 0.409 & 0.211 & 0.278 & 0.076 & 0.150 & 0.105 & 0.102 \\ code-audit & 56 & 0.421 & 0.211 & 0.281 & 0.072 & 0.139 & 0.094 & 0.090 \\ \bottomrule \end{tabular} \end{table}



% % \begin{table*}[t]
% % \centering
% % \caption{Results for the evaluated skills on the 266-case evaluation set.}
% % \label{tab:all_skill_metrics}
% % \scriptsize
% % \renewcommand{\arraystretch}{0.1}
% % \setlength{\tabcolsep}{3pt}
% % \begin{tabular*}{0.92\textwidth}{@{\extracolsep{\fill}}llrrrr}
% % \toprule
% % \textbf{Skill} & \textbf{Evaluation target} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{FPR} \\
% % \midrule
% % \multirow{4}{*}{vulnHunter}
% % & CWE attribution & 0.455 & 0.226 & 0.302 & 0.068 \\
% % & Vulnerable function localization & 0.184 & 0.184 & 0.184 & -- \\
% % & Vulnerable-line exact match & 0.086 & 0.086 & 0.086 & -- \\
% % & Vulnerable-statement exact match & 0.079 & 0.079 & 0.079 & -- \\
% % \midrule
% % \multirow{4}{*}{sast}
% % & CWE attribution & 0.361 & 0.162 & 0.223 & 0.071 \\
% % & Vulnerable function localization & 0.158 & 0.158 & 0.158 & -- \\
% % & Vulnerable-line exact match & 0.079 & 0.079 & 0.079 & -- \\
% % & Vulnerable-statement exact match & 0.064 & 0.064 & 0.064 & -- \\
% % \midrule
% % \multirow{4}{*}{Semgrep}
% % & CWE attribution & {} & {} & {} & {} \\
% % & Vulnerable function localization & {} & {} & {} & -- \\
% % & Vulnerable-line exact match & {} & {} & {} & -- \\
% % & Vulnerable-statement exact match & {} & {} & {} & -- \\
% % \midrule
% % \multirow{4}{*}{cybersecurity}
% % & CWE attribution & {} & {} & {} & {} \\
% % & Vulnerable function localization & {} & {} & {} & -- \\
% % & Vulnerable-line exact match & {} & {} & {} & -- \\
% % & Vulnerable-statement exact match & {} & {} & {} & -- \\
% % \midrule
% % \multirow{4}{*}{code-audit}
% % & CWE attribution & {} & {} & {} & {} \\
% % & Vulnerable function localization & {} & {} & {} & -- \\
% % & Vulnerable-line exact match & {} & {} & {} & -- \\
% % & Vulnerable-statement exact match & {} & {} & {} & -- \\
% % \midrule
% % \multirow{4}{*}{code-quality}
% % & CWE attribution & {} & {} & {} & {} \\
% % & Vulnerable function localization & {} & {} & {} & -- \\
% % & Vulnerable-line exact match & {} & {} & {} & -- \\
% % & Vulnerable-statement exact match & {} & {} & {} & -- \\
% % \midrule
% % \multirow{4}{*}{security-reviewer}
% % & CWE attribution & {} & {} & {} & {} \\
% % & Vulnerable function localization & {} & {} & {} & -- \\
% % & Vulnerable-line exact match & {} & {} & {} & -- \\
% % & Vulnerable-statement exact match & {} & {} & {} & -- \\
% % \midrule
% % \multirow{4}{*}{sast-configuration}
% % & CWE attribution & {} & {} & {} & {} \\
% % & Vulnerable function localization & {} & {} & {} & -- \\
% % & Vulnerable-line exact match & {} & {} & {} & -- \\
% % & Vulnerable-statement exact match & {} & {} & {} & -- \\
% % \bottomrule
% % \end{tabular*}
% % \end{table*}


==> tabs/qwen_discuss.tex <==
\begin{table*}[t]
\centering
\caption{Correctness rate (\%) on 100 new cases per skill and model.
Each pair reports baseline (B) $\rightarrow$ refined (R).
CWE: CWE correctness; Function: function localization;
F+S: joint function-and-statement localization;
Full: all three correct for the same finding.
Each $\Delta$ denotes the change from baseline to refined in percentage points.}
\label{tab:qwen-sif-test}

\scriptsize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{0.82}

\begin{tabular}{@{}l p{2.9cm} cc cc cc cc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multirow{2}{*}{\textbf{Skill}} &
\multicolumn{2}{c}{\textbf{CWE}} &
\multicolumn{2}{c}{\textbf{Function}} &
\multicolumn{2}{c}{\textbf{F+S}} &
\multicolumn{2}{c}{\textbf{Full}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
&
&
\textbf{B$\rightarrow$R} & $\boldsymbol{\Delta}$ &
\textbf{B$\rightarrow$R} & $\boldsymbol{\Delta}$ &
\textbf{B$\rightarrow$R} & $\boldsymbol{\Delta}$ &
\textbf{B$\rightarrow$R} & $\boldsymbol{\Delta}$ \\
\midrule

\multirow{5}{*}{Qwen3-Coder-Next (80B)}
& plugin-security-audit
& $11\rightarrow15$ & $+4$
& $7\rightarrow9$ & $+2$
& $4\rightarrow3$ & $-1$
& $3\rightarrow3$ & $0$ \\

& sickn33-differential-review
& $5\rightarrow7$ & $+2$
& $8\rightarrow6$ & $-2$
& $4\rightarrow2$ & $-2$
& $3\rightarrow0$ & $-3$ \\

& abstract-state-analyzer
& $7\rightarrow5$ & $-2$
& $6\rightarrow4$ & $-2$
& $3\rightarrow2$ & $-1$
& $2\rightarrow1$ & $-1$ \\

& anthropic-vuln-scan
& $4\rightarrow4$ & $0$
& $4\rightarrow7$ & $+3$
& $1\rightarrow2$ & $+1$
& $1\rightarrow2$ & $+1$ \\

& mcouthon-security-review
& $2\rightarrow3$ & $+1$
& $5\rightarrow3$ & $-2$
& $0\rightarrow0$ & $0$
& $0\rightarrow0$ & $0$ \\

\midrule

\multirow{5}{*}{Qwen3-Coder (480B)}
& plugin-security-audit
& $6\rightarrow5$ & $-1$
& $4\rightarrow3$ & $-1$
& $3\rightarrow2$ & $-1$
& $3\rightarrow1$ & $-2$ \\

& sickn33-differential-review
& $2\rightarrow1$ & $-1$
& $4\rightarrow4$ & $0$
& $2\rightarrow1$ & $-1$
& $1\rightarrow0$ & $-1$ \\

& abstract-state-analyzer
& $6\rightarrow7$ & $+1$
& $5\rightarrow3$ & $-2$
& $3\rightarrow2$ & $-1$
& $3\rightarrow2$ & $-1$ \\

& anthropic-vuln-scan
& $3\rightarrow4$ & $+1$
& $4\rightarrow4$ & $0$
& $0\rightarrow0$ & $0$
& $0\rightarrow0$ & $0$ \\

& mcouthon-security-review
& $3\rightarrow2$ & $-1$
& $1\rightarrow2$ & $+1$
& $1\rightarrow1$ & $0$
& $1\rightarrow0$ & $-1$ \\

\midrule

\multirow{5}{*}{Qwen3-Coder-30B}
& plugin-security-audit
& $7\rightarrow8$ & $+1$
& $2\rightarrow2$ & $0$
& $1\rightarrow2$ & $+1$
& $1\rightarrow2$ & $+1$ \\

& sickn33-differential-review
& $2\rightarrow0$ & $-2$
& $4\rightarrow5$ & $+1$
& $0\rightarrow1$ & $+1$
& $0\rightarrow0$ & $0$ \\

& abstract-state-analyzer
& $0\rightarrow1$ & $+1$
& $1\rightarrow1$ & $0$
& $0\rightarrow0$ & $0$
& $0\rightarrow0$ & $0$ \\

& anthropic-vuln-scan
& $2\rightarrow5$ & $+3$
& $2\rightarrow4$ & $+2$
& $1\rightarrow0$ & $-1$
& $1\rightarrow0$ & $-1$ \\

& mcouthon-security-review
& $0\rightarrow2$ & $+2$
& $2\rightarrow2$ & $0$
& $0\rightarrow1$ & $+1$
& $0\rightarrow1$ & $+1$ \\

\bottomrule
\end{tabular}
\end{table*}

==> tabs/skill-performance.tex <==
\begin{table}[t]
\centering
\caption{Top-5 performing skills}
\label{tab:skill_performance}
% \begin{tabular}{lcl}
\begin{tabular}{lc}
\toprule
\textbf{Skill} & \textbf{Correct / 400} 
% & \textbf{Observed Strength} 
\\
\midrule
\texttt{plugin-security-audit}
& 63 (15.75\%)

% & Broad exploration and reconstruction of multi-step execution dependencies 
\\

\texttt{sickn33-differential-review}
& 62 (15.50\%)
% & Contextual analysis of helper effects and state changes across related code
\\

\texttt{abstract-state-analyzer}
& 60 (15.00\%)
% & Systematic tracking of ranges, state values, and local invariants 
\\

\texttt{anthropic-vuln-scan}
& 60 (15.00\%)
% & Strong conversion from relevant-function discovery to complete localized findings 
\\

\texttt{mcouthon-security-review}
& 58 (14.50\%)
% & Cross-function ownership, caller analysis, and distinction between related object lifetimes 
\\
\bottomrule
\end{tabular}
\end{table}

==> tabs/skills.tex <==
% \begin{table*}[t]
% \centering
% \caption{The Final Selected Skills}
% \label{tab:skills}
% \scriptsize
% \begin{tabular}{p{0.23\textwidth}p{0.14\textwidth}p{0.55\textwidth}}
% \hline
% \textbf{Workflow/process pattern} & \textbf{Representative} & \textbf{Native task and expected evidence} \\
% \hline
% Automated security scanning & \href{https://github.com/trailofbits/skills/blob/main/plugins/static-analysis/skills/semgrep/SKILL.md}{Semgrep} & Execute a pinned static-analysis engine and rules; preserve scanner command and machine-readable findings. \\
% Security-scanning governance & \href{https://github.com/wshobson/agents/blob/main/plugins/security-scanning/skills/sast-configuration/SKILL.md}{sast-configuration} & Design tool/rule selection, exclusions, baselining, suppressions, quality gates, ownership, and CI policy from a governance brief. \\
% Vulnerability variant discovery & \href{https://github.com/sendaifun/skills/blob/main/skills/vulnhunter/SKILL.md}{vulnhunter} & Generalize an independently supplied seed root cause, search the repository, and validate or reject variants. \\
% Source-to-sink data-flow review & \href{https://github.com/H-mmer/pentest-agents/blob/main/providers/codex/.agents/skills/sast/SKILL.md}{sast} & Trace attacker-controlled or invalid state to a security-sensitive sink and report the enabling missing check or invariant. \\
% Multi-agent security audit & \href{https://github.com/AgriciDaniel/claudecybersecurity/blob/main/skills/cybersecurity/SKILL.md}{cybersecurity} & Decompose the audit among specialist agents, synthesize their evidence, and resolve conflicting findings. \\
% Specification-compliance review & \href{https://github.com/WenJunDuan/Rlues/blob/main/vibeCoding/old%20version/config-agent_v8.2/.claude/skills/code-quality/SKILL.md}{code-quality} & Compare implementation evidence against an independent specification or plan and report compliant, violated, and unverified requirements. \\
% Structured code security review & \href{https://github.com/Jeffallan/claude-skills/blob/main/skills/security-reviewer/SKILL.md}{security-reviewer} & Follow a systematic review checklist and produce localized, prioritized source findings. \\
% Threat-modeled security audit & \href{https://github.com/3stoneBrother/code-audit/blob/main/SKILL.md}{code-audit} & Establish assets, trust boundaries, entry points, and plausible attack paths before producing a focused code finding. \\
% \hline
% \end{tabular}
% \end{table*}


==> tabs/taxonomy.tex <==
% \begin{table}[t]
% \centering
% \caption{Root-cause taxonomy frequencies. Labels are multi-label and can overlap.}
% \label{tab:root-cause-summary}
% \scriptsize
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lc}
% \toprule
% Root cause & Count \\
% \midrule
% RC1: Shallow Pattern Matching&  \\
% RC2: Incomplete Vulnerability Evidence Chain &  \\
% RC3: Incomplete Code-Context Reasoning &  \\
% RC4: Insufficient Workflow Enforcement &  \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

==> tabs/vul_classes_det.tex <==
\begin{table}[t]
\centering
\caption{Exact CWE match by vulnerability class.}
\label{tab:cwe-class-results}
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{lccccc}
\toprule
Skill & CWE-476 & CWE-416 & CWE-125 & CWE-787 & CWE-120 \\
\midrule
vulnHunter & 40/115 & 9/88 & 6/34 & 5/28 & 0/1 \\
Semgrep & 46/115 & 7/88 & 6/34 & 8/28 & 0/1 \\
code-quality & 39/115 & 10/88 & 6/34 & 6/28 & 0/1 \\
sast & 26/115 & 12/88 & 3/34 & 1/28 & 1/1 \\
sast-configuration & 41/115 & 15/88 & 5/34 & 2/28 & 0/1 \\
security-reviewer & 40/115 & 8/88 & 7/34 & 5/28 & 0/1 \\
cybersecurity & 32/115 & 10/88 & 9/34 & 5/28 & 0/1 \\
code-audit & 36/115 & 9/88 & 7/34 & 4/28 & 0/1 \\
\bottomrule
\end{tabular}%

\end{table}
